Improvement and Renormalization Constants in O(a) Improved Lattice QCD

We present results at beta=6.0 and 6.2 for the O(a) improvement and renormalization constants for bilinear operators using axial and vector Ward identities. We discuss the extraction of the mass dependence of the renormalization constants and the coefficients of the equation of motion operators.

==> Makefile <==
# %auto-ignore
MAINFILE=  paper.tex

TEXFILES=  tabfinal.tex tabcprime.tex

AXISFILES= 

FIGFILES=  
PSFILES=   
#########################################################################
# special rules if any

#########################################################################
#									#
#                 NO USER SERVICEABLE PARTS BELOW !!!                   #
# 									#
#########################################################################


# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${PSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps} ${PSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create ps.
%.ps: %.fig
	fig2dev -L ps $< > $@

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | /usr/local/bin/plot2ps > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" -e 's/useclippath true def/useclippath false def/' \
	$@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | /usr/local/bin/plot2ps > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" -e 's/useclippath true def/useclippath false def/' \
	$@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<

%.ps2: %.ps
	pstops -w21cm -h29.7cm '2:0L@.65(1w,0)+1L@.65(1w,.5h)' $< | sed -e '1a\
	%%Orientation: Landscape' > $@

# dvi is always created from tex.
%.dvi: %.tex
	latex $<
	if grep -i -q rerun ${<:.tex=.log} ; then latex $<; fi

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS}" ; \
	 echo "submission") | uufiles -gz -9

